Harder or Different? Understanding Generalization of Audio Deepfake Detection

Recent research has highlighted a key issue in speech deepfake detection: models trained on one set of deepfakes perform poorly on others. The question arises: is this due to the continuously improving quality of Text-to-Speech (TTS) models, i.e., are newer DeepFakes just 'harder' to detect? Or, is it because deepfakes generated with one model are fundamentally different to those generated using another model? We answer this question by decomposing the performance gap between in-domain and out-of-domain test data into 'hardness' and 'difference' components. Experiments performed using ASVspoof databases indicate that the hardness component is practically negligible, with the performance gap being attributed primarily to the difference component. This has direct implications for real-world deepfake detection, highlighting that merely increasing model capacity, the currently-dominant research trend, may not effectively address the generalization challenge.

==> res/tab/asv19_vs_21.tex <==
\begin{tabular}{lllrrr}
\toprule
Model Name & Training Data & Test Data &  Performance Gap &  Hardness Gap &  Difference Gap \\
\midrule
   rawnet2 &         asv19 &  asv21\_la &       -17.539343 &     -3.911512 &      -13.627831 \\
   rawnet2 &         asv19 &  asv21\_df &       -20.212690 &     -0.804733 &      -19.407957 \\
  ssl\_w2v2 &         asv19 &  asv21\_la &        -6.278601 &     -0.663533 &       -5.615068 \\
  ssl\_w2v2 &         asv19 &  asv21\_df &        -3.397253 &     -0.123992 &       -3.273261 \\
 lcnn\_wang &         asv19 &  asv21\_la &       -19.943986 &     -7.379286 &      -12.564700 \\
 lcnn\_wang &         asv19 &  asv21\_df &       -17.464347 &     -0.175084 &      -17.289264 \\
\bottomrule
\end{tabular}

==> res/tab/ex2/audiomentations.tex <==

\begin{tabular}{lll|l|lll}
\toprule
Model Name &       Training Data &              Test Data &       Test eer & Performance Gap & Hardness Gap & Difference Gap \\
\midrule
 lcnn wang & audiomentations.p=0 &    audiomentations.p=0 &  $3.8 \pm 3.0$ &     $0.1 \pm 4$ & $-0.0 \pm 4$ &    $0.1 \pm 4$ \\
 % lcnn wang & audiomentations.p=0 &  audiomentations.p=0.1 &  $5.9 \pm 3.1$ &     $2.2 \pm 4$ & $-1.1 \pm 3$ &    $3.3 \pm 3$ \\
 % lcnn wang & audiomentations.p=0 & audiomentations.p=0.25 &  $9.6 \pm 3.4$ &     $5.9 \pm 4$ & $-0.0 \pm 3$ &    $5.9 \pm 3$ \\
 lcnn wang & audiomentations.p=0 &  audiomentations.p=0.5 & $15.1 \pm 3.4$ &    $11.4 \pm 4$ &  $2.9 \pm 3$ &    $8.5 \pm 3$ \\
 lcnn wang & audiomentations.p=0 &    audiomentations.p=1 & $25.1 \pm 5.5$ &    $21.4 \pm 6$ &  $6.0 \pm 3$ &   $15.5 \pm 6$ \\
  \midrule
   rawnet2 & audiomentations.p=0 &    audiomentations.p=0 &  $6.5 \pm 1.6$ &     $0.1 \pm 2$ & $-0.0 \pm 2$ &    $0.1 \pm 2$ \\
   % rawnet2 & audiomentations.p=0 &  audiomentations.p=0.1 &  $8.0 \pm 1.7$ &     $1.5 \pm 2$ &  $0.9 \pm 2$ &    $0.6 \pm 2$ \\
   % rawnet2 & audiomentations.p=0 & audiomentations.p=0.25 & $10.3 \pm 1.0$ &     $3.9 \pm 2$ &  $4.3 \pm 3$ &   $-0.5 \pm 3$ \\
   rawnet2 & audiomentations.p=0 &  audiomentations.p=0.5 & $13.5 \pm 1.2$ &     $7.1 \pm 2$ &  $2.7 \pm 2$ &    $4.4 \pm 2$ \\
   rawnet2 & audiomentations.p=0 &    audiomentations.p=1 & $20.2 \pm 2.5$ &    $13.7 \pm 3$ & \cellcolor{blue!25} $12.8 \pm 2$ &   \cellcolor{blue!25} $0.9 \pm 3$ \\
  \midrule
  ssl w2v2 & audiomentations.p=0 &    audiomentations.p=0 &  $0.2 \pm 0.1$ &     $0.0 \pm 0$ & $-0.0 \pm 0$ &    $0.0 \pm 0$ \\
  % ssl w2v2 & audiomentations.p=0 &  audiomentations.p=0.1 &  $1.9 \pm 0.2$ &     $1.7 \pm 0$ &  $0.9 \pm 0$ &    $0.8 \pm 0$ \\
  % ssl w2v2 & audiomentations.p=0 & audiomentations.p=0.25 &  $4.4 \pm 0.4$ &     $4.2 \pm 0$ &  $0.9 \pm 0$ &    $3.3 \pm 0$ \\
  ssl w2v2 & audiomentations.p=0 &  audiomentations.p=0.5 &  $7.6 \pm 1.1$ &     $7.4 \pm 1$ &  $1.7 \pm 1$ &    $5.7 \pm 1$ \\
  ssl w2v2 & audiomentations.p=0 &    audiomentations.p=1 & $12.6 \pm 0.8$ &    $12.4 \pm 1$ &  $2.3 \pm 0$ &   $10.1 \pm 1$ \\
  \midrule
 whisperdf & audiomentations.p=0 &    audiomentations.p=0 &  $0.3 \pm 0.1$ &    $-0.0 \pm 0$ & $-0.0 \pm 0$ &   $-0.0 \pm 0$ \\
 whisperdf & audiomentations.p=0 &  audiomentations.p=0.1 &  $2.2 \pm 0.3$ &     $1.8 \pm 0$ &  $1.2 \pm 0$ &    $0.6 \pm 0$ \\
 % whisperdf & audiomentations.p=0 & audiomentations.p=0.25 &  $4.8 \pm 0.9$ &     $4.4 \pm 1$ &  $1.6 \pm 0$ &    $2.8 \pm 1$ \\
 % whisperdf & audiomentations.p=0 &  audiomentations.p=0.5 &  $8.1 \pm 0.5$ &     $7.8 \pm 1$ &  $2.1 \pm 0$ &    $5.6 \pm 1$ \\
 whisperdf & audiomentations.p=0 &    audiomentations.p=1 & $13.4 \pm 0.8$ &    $13.0 \pm 1$ &  $3.1 \pm 1$ &    $9.8 \pm 1$ \\
\bottomrule
\end{tabular}

==> res/tab/ex2/background_music_or_noise.tex <==
\begin{tabular}{lll|l|lll}
\toprule
Model Name &                     Training Data &                            Test Data & Test EER & Performance Gap & Hardness Gap & Difference Gap \\
\midrule
 lcnn wang & add background music or noise.p=0 &    add background music or noise.p=0 &    $1.9 \pm 0.2$ &     $0.1 \pm 0$ & $-0.0 \pm 0$ &    $0.1 \pm 0$ \\
 % lcnn wang & add background music or noise.p=0 &  add background music or noise.p=0.1 &    $3.3 \pm 0.3$ &     $1.4 \pm 0$ &  $1.4 \pm 1$ &    $0.1 \pm 1$ \\
 % lcnn wang & add background music or noise.p=0 & add background music or noise.p=0.25 &    $5.9 \pm 0.9$ &     $4.1 \pm 1$ &  $1.6 \pm 0$ &    $2.5 \pm 1$ \\
 lcnn wang & add background music or noise.p=0 &  add background music or noise.p=0.5 &   $10.4 \pm 1.5$ &     $8.6 \pm 2$ &  $3.7 \pm 1$ &    $4.8 \pm 2$ \\
 lcnn wang & add background music or noise.p=0 &    add background music or noise.p=1 &   $18.5 \pm 2.7$ &    $16.6 \pm 3$ &  $4.7 \pm 3$ &   $11.9 \pm 4$ \\
  \midrule
   rawnet2 & add background music or noise.p=0 &    add background music or noise.p=0 &    $6.6 \pm 0.7$ &     $0.0 \pm 1$ & $-0.0 \pm 1$ &    $0.0 \pm 1$ \\
   % rawnet2 & add background music or noise.p=0 &  add background music or noise.p=0.1 &    $7.0 \pm 0.9$ &     $0.5 \pm 1$ &  $0.1 \pm 2$ &    $0.4 \pm 2$ \\
   % rawnet2 & add background music or noise.p=0 & add background music or noise.p=0.25 &    $8.0 \pm 1.3$ &     $1.5 \pm 2$ & $-0.5 \pm 1$ &    $2.0 \pm 1$ \\
   rawnet2 & add background music or noise.p=0 &  add background music or noise.p=0.5 &    $9.1 \pm 1.1$ &     $2.5 \pm 1$ &  $0.5 \pm 4$ &    $2.1 \pm 4$ \\
   rawnet2 & add background music or noise.p=0 &    add background music or noise.p=1 &   $10.9 \pm 1.7$ &     $4.4 \pm 2$ &  $4.0 \pm 1$ &    $0.4 \pm 2$ \\
  \midrule
  ssl w2v2 & add background music or noise.p=0 &    add background music or noise.p=0 &    $0.3 \pm 0.0$ &    $-0.0 \pm 0$ & $-0.0 \pm 0$ &   $-0.0 \pm 0$ \\
  % ssl w2v2 & add background music or noise.p=0 &  add background music or noise.p=0.1 &    $1.1 \pm 0.3$ &     $0.8 \pm 0$ &  $0.3 \pm 0$ &    $0.5 \pm 0$ \\
  % ssl w2v2 & add background music or noise.p=0 & add background music or noise.p=0.25 &    $2.0 \pm 0.2$ &     $1.8 \pm 0$ &  $0.1 \pm 0$ &    $1.6 \pm 0$ \\
  ssl w2v2 & add background music or noise.p=0 &  add background music or noise.p=0.5 &    $3.0 \pm 0.8$ &     $2.7 \pm 1$ &  $0.0 \pm 0$ &    $2.7 \pm 1$ \\
  ssl w2v2 & add background music or noise.p=0 &    add background music or noise.p=1 &    $4.9 \pm 0.9$ &     $4.6 \pm 1$ &  $0.2 \pm 0$ &    $4.4 \pm 1$ \\
  \midrule
 whisperdf & add background music or noise.p=0 &    add background music or noise.p=0 &    $0.4 \pm 0.0$ &    $-0.0 \pm 0$ & $-0.0 \pm 0$ &   $-0.0 \pm 0$ \\
 % whisperdf & add background music or noise.p=0 &  add background music or noise.p=0.1 &    $1.1 \pm 0.1$ &     $0.7 \pm 0$ &  $0.2 \pm 0$ &    $0.5 \pm 0$ \\
 % whisperdf & add background music or noise.p=0 & add background music or noise.p=0.25 &    $1.7 \pm 0.3$ &     $1.2 \pm 0$ &  $0.5 \pm 1$ &    $0.8 \pm 1$ \\
 whisperdf & add background music or noise.p=0 &  add background music or noise.p=0.5 &    $2.8 \pm 0.6$ &     $2.4 \pm 1$ &  $0.4 \pm 0$ &    $2.0 \pm 1$ \\
 whisperdf & add background music or noise.p=0 &    add background music or noise.p=1 &    $4.6 \pm 0.7$ &     $4.2 \pm 1$ &  $1.0 \pm 0$ &    $3.2 \pm 1$ \\
\bottomrule
\end{tabular}

==> res/v2/exp0/delta=0.005_Patience=5/asv19train_vs_eval.tex <==
\begin{tabular}{llll}
\toprule
Model Name & Performance Gap &  Hardness Gap & Difference Gap \\
\midrule
   rawnet2 &    $13.8 \pm 2$ &   $2.3 \pm 3$ &   $11.5 \pm 4$ \\
  ssl_w2v2 &    $21.3 \pm 3$ & $0.1 \pm nan$ & $21.2 \pm nan$ \\
 whisperdf &    $14.5 \pm 3$ &   $0.1 \pm 0$ &   $14.4 \pm 3$ \\
 lcnn_wang &    $20.8 \pm 5$ & $0.3 \pm nan$ & $20.5 \pm nan$ \\
\bottomrule
\end{tabular}

==> res/v2/exp0/delta=0.005_patience=2/asv19train_vs_eval.tex <==
\begin{tabular}{llll}
\toprule
Model Name & Performance Gap & Hardness Gap & Difference Gap \\
\midrule
 whisperdf &    $12.4 \pm 2$ &  $0.4 \pm 0$ &   $12.0 \pm 2$ \\
   rawnet2 &    $12.8 \pm 2$ &  $5.4 \pm 1$ &    $7.4 \pm 2$ \\
 lcnn_wang &   $16.7 \pm 11$ & $9.2 \pm 18$ &   $7.5 \pm 21$ \\
  ssl_w2v2 &    $15.4 \pm 8$ &  $0.2 \pm 0$ &   $15.1 \pm 8$ \\
\bottomrule
\end{tabular}

==> res/v2/exp0/delta=0.05_patience=2/asv19train_vs_eval.tex <==
\begin{tabular}{llll}
\toprule
Model Name & Performance Gap &   Hardness Gap & Difference Gap \\
\midrule
 whisperdf &     $9.3 \pm 1$ &    $1.2 \pm 1$ &    $8.1 \pm 1$ \\
   rawnet2 &    $14.1 \pm 2$ &    $2.3 \pm 2$ &   $11.9 \pm 2$ \\
 lcnn_wang &   $16.5 \pm 10$ &    $1.0 \pm 1$ &  $15.5 \pm 10$ \\
  ssl_w2v2 &   $16.5 \pm 17$ & $-1.3 \pm nan$ & $17.9 \pm nan$ \\
\bottomrule
\end{tabular}

==> res/v2/exp2/gaussian_noise.tex <==
\begin{tabular}{lllllll}
\toprule
Model Name &       Training Data &              Test Data &      Test eer & Performance Gap & Hardness Gap & Difference Gap \\
\midrule
   rawnet2 & audiomentations.p=0 &    audiomentations.p=0 & $2.4 \pm 0.9$ &     $0.0 \pm 1$ & $-0.0 \pm 1$ &    $0.0 \pm 1$ \\
   rawnet2 & audiomentations.p=0 & audiomentations.p=0.25 & $3.4 \pm 0.6$ &     $1.1 \pm 1$ &  $0.5 \pm 1$ &    $0.6 \pm 1$ \\
   rawnet2 & audiomentations.p=0 &  audiomentations.p=0.5 & $4.3 \pm 1.3$ &     $2.0 \pm 2$ &  $1.6 \pm 2$ &    $0.3 \pm 2$ \\
   rawnet2 & audiomentations.p=0 &    audiomentations.p=1 & $5.6 \pm 1.6$ &     $3.3 \pm 2$ &  $1.0 \pm 1$ &    $2.3 \pm 2$ \\
  ssl_w2v2 & audiomentations.p=0 &    audiomentations.p=0 & $0.3 \pm 0.0$ &    $-0.0 \pm 0$ & $-0.0 \pm 0$ &   $-0.0 \pm 0$ \\
  ssl_w2v2 & audiomentations.p=0 & audiomentations.p=0.25 & $1.1 \pm 0.3$ &     $0.8 \pm 0$ &  $0.0 \pm 0$ &    $0.8 \pm 0$ \\
  ssl_w2v2 & audiomentations.p=0 &  audiomentations.p=0.5 & $1.9 \pm 0.6$ &     $1.6 \pm 1$ &  $0.1 \pm 0$ &    $1.5 \pm 1$ \\
  ssl_w2v2 & audiomentations.p=0 &    audiomentations.p=1 & $3.2 \pm 1.0$ &     $2.9 \pm 1$ &  $0.6 \pm 1$ &    $2.3 \pm 1$ \\
 whisperdf & audiomentations.p=0 &    audiomentations.p=0 & $0.4 \pm 0.0$ &    $-0.0 \pm 0$ & $-0.0 \pm 0$ &   $-0.0 \pm 0$ \\
 whisperdf & audiomentations.p=0 & audiomentations.p=0.25 & $2.3 \pm 0.9$ &     $1.9 \pm 1$ &  $0.5 \pm 0$ &    $1.4 \pm 1$ \\
 whisperdf & audiomentations.p=0 &  audiomentations.p=0.5 & $3.8 \pm 1.2$ &     $3.4 \pm 1$ &  $0.8 \pm 0$ &    $2.6 \pm 1$ \\
 whisperdf & audiomentations.p=0 &    audiomentations.p=1 & $6.7 \pm 1.4$ &     $6.2 \pm 1$ &  $1.6 \pm 1$ &    $4.6 \pm 1$ \\
\bottomrule
\end{tabular}

==> results_table_3_4.tex <==
\begin{table*}[ht]
    \centering
    % \resizebox{.5\textwidth}{!}{
    %     \input{res/tab/asv21la}
    % }
    \begin{tabular}{lllllll}
\toprule
&&\multicolumn{2}{l}{\textbf{Results on ASVspoof21} DF}&&\multicolumn{2}{l}{\textbf{Results on In-the-wild}}\\ \cline{2-7}
Model Name & Performance Gap & Hardness Gap & Difference Gap&Performance Gap & Hardness Gap & Difference Gap \\
\midrule
LCNN Wang &    $26.6 \pm 3$ &  $1.7 \pm 2$ &   $25.0 \pm 3$ & $78.2 \pm 15$&$-1.5 \pm 2$&$79.7 \pm 15$ \\
RawNet2 &    $18.1 \pm 7$ & $-2.2 \pm 7$ &   $20.3 \pm 2$& $40.6 \pm 7$& $-6.4 \pm 7$&$47.0 \pm 3$ \\
SSL W2V2 &    $14.2 \pm 3$ &  $0.1 \pm 0$ &   $14.0 \pm 3$ & $30.3 \pm 5$ &  $0.1 \pm 0$& $30.2 \pm 5$\\
WhisperDF &    $15.2 \pm 2$ &  $0.1 \pm 0$ &   $15.1 \pm 2$& $31.4 \pm 5$ & $-0.5 \pm 0$& $31.9 \pm 5$ \\
\bottomrule
\end{tabular}
    \caption{Decomposition of the performance gap when training on ASVspoof 19 and evaluating on ASVspoof 21 and In-the-Wild. }
    \label{tab:ASVspoof21DF_ITW}
\end{table*}

